Meili: Enabling SmartNIC as a Service in the Cloud

SmartNICs are touted as an attractive substrate for network application offloading, offering benefits in programmability, host resource saving, and energy efficiency. The current usage restricts offloading to local hosts and confines SmartNIC ownership to individual application teams, resulting in poor resource efficiency and scalability. This paper presents Meili, a novel system that realizes SmartNIC as a service to address these issues. Meili organizes heterogeneous SmartNIC resources as a pool and offers a unified one-NIC abstraction to application developers. This allows developers to focus solely on the application logic while dynamically optimizing their performance needs. Our evaluation on NVIDIA BlueField series and AMD Pensando SmartNICs demonstrates that Meili achieves scalable single-flow throughput with a maximum 8 {\mu}s latency overhead and enhances resource efficiency by 3.07$\times$ compared to standalone deployments and 1.44$\times$ compared to state-of-the-art microservice deployments.

==> Makefile <==
DOCUMENT=main

default: $(DOCUMENT).pdf

$(DOCUMENT).toc: $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

$(DOCUMENT).pdf: $(DOCUMENT).toc
	bibtex $(DOCUMENT)
	pdflatex $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

all: $(DOCUMENT).pdf

clean:
	rm -rf *.aux $(DOCUMENT).log $(DOCUMENT).toc \
     $(DOCUMENT).bbl $(DOCUMENT).blg *.bak \
		 $(DOCUMENT).out *.log *.gz\
      $(DOCUMENT).pdf *.fls *.fdb_latexmk

open:
	open $(DOCUMENT).pdf

gopen:
	gnome-open $(DOCUMENT).pdf

opens:
	open $(DOCUMENT).tex

gopens:
	gnome-open $(DOCUMENT).tex


